Help, Anna! Visual Navigation with Natural Multimodal Assistance via Retrospective Curiosity-Encouraging Imitation Learning

Mobile agents that can leverage help from humans can potentially accomplish more complex tasks than they could entirely on their own. We develop "Help, Anna!" (HANNA), an interactive photo-realistic simulator in which an agent fulfills object-finding tasks by requesting and interpreting natural language-and-vision assistance. An agent solving tasks in a HANNA environment can leverage simulated human assistants, called ANNA (Automatic Natural Navigation Assistants), which, upon request, provide natural language and visual instructions to direct the agent towards the goals. To address the HANNA problem, we develop a memory-augmented neural agent that hierarchically models multiple levels of decision-making, and an imitation learning algorithm that teaches the agent to avoid repeating past mistakes while simultaneously predicting its own chances of making future progress. Empirically, our approach is able to ask for help more effectively than competitive baselines and, thus, attains higher task success rate on both previously seen and previously unseen environments. We publicly release code and data at https://github.com/khanhptnk/hanna . A video demo is available at https://youtu.be/18P94aaaLKg .

==> sections/env.tex <==
\paragraph{Simulator.} The Matterport3D dataset (CITE Matterport) is a large RGB-D dataset for scene understanding in indoor environments. It contains 10,800 panoramic views inside 90 real building-scale scenes, constructed from 194,400 RGBD
images. Each scene is residential building consisting of multiple rooms and floor levels, and is annotated with surface
constructions, camera poses, and semantic segmentations. Using this dataset, (CITE Anderson et al) implemented a simulator that
emulates an agent walking in indoor environments. Navigation is accomplished by traversing edges in pre-defined environment graphs whose edges connect locations that are reachable within five meters.

\paragraph{Language-based recovery routes.} The Matterport3D simulator is accompanied by a dataset called Room-to-Room (CITE), intended for teaching agents to navigate to random locations in indoor environments by following natural language navigation instructions. 
Language diversity is captured; each navigation path is associated with three different instructions. 
In total, the dataset contains 21,567 instructions with an average length of 29 words, featuring 7,189 paths with an average path length of 10m. 
We utilize the Room-to-Room dataset to setup \system in the Matterport3D environments.
Some filters. 
Some stats. 



==> sections/framework.tex <==
\subsection{Preliminaries}
We consider an agent living in a stochastic partially-observable environment $\mathcal{E} = (\mathcal{S}, \mathcal{Z}, \mathcal{A}, \mathcal{T}, \mathcal{O})$ defined by an environment state space $\mathcal{S}$, a observation state space $\mathcal{Z}$, an action space $\mathcal{A}$, a transition function $\mathcal{T}: \mathcal{S} \times \mathcal{A} \rightarrow [0, 1]^{|\mathcal{S}|}$, and an observation function $\mathcal{O}: \mathcal{S} \times \mathcal{A} \rightarrow [0, 1]^{|\mathcal{Z}|}$.
The agent is regarded as part of the environment, thus the states $s \in \mathcal{S}$ also capture its internal states (any essential information that the agent keeps track of).
$\mathcal{T}(s, a, s')$ represents the probability that state $s'$ follows state $s$ after the action $a$ is taken. 
$\mathcal{O}(s, a, z)$ defines the probability that the agent observes $z$ after taking $a$ and transitioning to state $s'$.
They agent does not have access to environment states and only makes decisions based on observations.

In this environment, the agent is requested to perform a task $\tau = \left(c, s_{\textrm{start}}, \beta^{\star} \right)$, defined by a task command $c$, a start state $s_{\textrm{start}}$, and a termination function $\beta^{\star}:\mathcal{S} \rightarrow \{0, 1\}$. 
The task requires the agent to start at state $s_{\textrm{start}}$, process the command $c$ and execute a sequence of actions that leads to any goal state $s \in \mathcal{S}_{\textrm{goal}} = \{s \in \mathcal{S} : \beta^{\star}(s) = 1\}$.
The termination function is not given to the agent during the task execution. 
For our interest, we focus on task commands specified via language. 
We consider the general case when the task requester may \emph{not} know in advance how to accomplish the task.
Hence, the task command may only describe the end-goal of the task and not the detailed sequential steps to execute it (e.g, ``Find a cup"). 

The task command persists throughout the task execution as part of the environment observed by the agent.
To capture this aspect, we define the task-augmented environment $\mathcal{E}_{\tau} = (\mathcal{S}_{\tau}, \mathcal{Z}_{\tau}, \mathcal{A}, \mathcal{T}_{\tau}, \mathcal{O}_{\tau})$, of which the states $s \in \mathcal{S}_{\tau}$ and observations $z \in \mathcal{Z}_{\tau}$ augment the original state and observation representations with a representation of the task command.  
To perform the task, the agent maintains an execution policy $\pi: \mathcal{Z}_{\tau} \times \mathcal{A} \rightarrow [0, 1]^{|\mathcal{A}|}$ and a termination policy $\beta: \mathcal{Z}_{\tau} \rightarrow [0, 1]^2$.
At time step $t$, the agent receives an observation $z_t$ and takes an action $a_t^{\textrm{term}} \mapsfrom \beta(z_t)$\footnote{We use the notation $a \mapsfrom f(z)$ to denote an action selected according to a process from the action distribution computed by a policy $f$ on the observation $z$. The process, which is usually taking $\arg\max$ or sampling, will be clearly described in our implementation.} to decide whether it wants to continue the task execution. 
If $a_t^{\textrm{term}} = 0$, the agent selects an action $a_t \mapsfrom \pi(z_t)$, which transitions it to the next state $s_{t + 1} \sim \mathcal{T}_{\tau}(s_t, a_t)$.
The new observation $z_{t + 1} \sim \mathcal{O}_{\tau}(s_{t + 1}, a_t)$ is sent to agent in the next step. 
If $a_t^{\textrm{term}} = 1$, the agent stops executing the task. 

\subsection{Human Assistance via Intervention}

During executing a task, the agent may get lost and become unable to make progress. 
To help the agent recover in those situations, we introduce into the environment an assistant $\Phi$.
We assume that the assistant is generally better than the agent at performing the task.
For example, it can be a human who is familiar with the environment or a virtual automatic assistant that monitors the environment. 
We define the recovery state set $\mathcal{S}_{\Phi} \subseteq \mathcal{S}$ as the set of states where the agent can request help from the assistant.
Restricting the recovery states captures the fact that the assistant is not always available or willing to help the agent. 
For example, a human may not be interested in finding the agent all the time and only provide help when it is nearby; a virtual assistance system may have difficulties locating the agent in a complex environment and can only detect the agent at certain locations. 
The agent actively seeks for help by going to the recovery states. 
To decide when it needs additional assistance, the agent maintains a help-requesting policy $\askpol: \mathcal{S} \rightarrow [0, 1]^2$. 
At time step $t$, the agent selects an action $a_t^{\textrm{ask}} \mapsfrom \askpol(z_t)$. 
Obviously, $a_t^{\textrm{ask}} = 0$ if the current state is a non-recovery state ($s_t \notin \mathcal{S}_{\Phi}$).
If $a_t^{\textrm{ask}} = 1 $, the agent signals the assistant for help.

Upon requested, the assistant replies the agent with an intervention whose goal is to improve the agent's current situation by directing it to take a sequence of actions.
We consider two types of intervention: \emph{direct} and \emph{indirect}. 
When the assistant intervenes directly, the agent lets the assistant take control and make decisions on its behalf. 
In contrast, in the case of indirect intervention, the assistant alters the environment to influence the agent's decisions. 
The distinction between direct and indirect intervention is illustrated more tangibly in a physical agent such as a self-driving car. 
In this case, turning off the automatic driving mode and taking control of the steering wheel represents a direct intervention, whereas issuing a language command to slow down the car or making an unpleasant face gesture to signal the car to drive more comfortably are examples of indirect intervention. 
As seen from this example, the notion of ``altering the environment" of indirect intervention does not necessarily imply major changes to the environment structure (e.g., build a new road), but can be as simple as injecting extra information to manipulate the agent's internal state. 
In this point of view, assistance via human-intelligible media (e.g., words, images, body gestures) is categorized as indirect intervention. 

\subsection{Intervention as Environment-aware Option}

CITE introduce the notion of option to represent a temporally extended course of actions.
Options are building blocks of hierarchical reinforcement learning and imitation learning, serving as high-level actions or subtasks (CITE).
Formally, a (conventional) option $o = (\mathcal{I}_o, \pi_o, \beta_o)$ is defined by a initiation set of states $\mathcal{I}_o \subseteq \mathcal{S}$ where the option is available, an execution policy $\pi_o : \mathcal{Z} \rightarrow [0, 1]^{|\mathcal{A}|}$, and a termination function $\beta_o: \mathcal{S} \rightarrow \{0, 1\}$.
At a state $s \in \mathcal{I}_o$, if the agent chooses to take the option, it will follow decisions made by $\pi_o$ until reaching a state $s'$ where $\beta(s') = 1$.
For example, an option ``open-a-door" is a sequence of (primitive) actions to locate the doorknob, turn and hold it to open the door. 


To model intervention precisely, we present a natural extension of the conventional option, called \emph{environment-aware option}. 
An environment-aware option $o = (\mathcal{E}_o, \mathcal{I}_o, \pi_o, \beta_o)$ specifies the environment $\mathcal{E}_o = (\mathcal{I}_o, \mathcal{Z}_o, \mathcal{A}, \mathcal{T}_o, \mathcal{O}_o)$ in which the option's execution policy and termination function make decisions. 
The policies $\pi_o$ and $\beta_o$ takes input from $S_o$, and queries $\mathcal{T}_o$ and $\mathcal{O}_o$ to transition to new states.
Specifying the option environment is crucial to reflect the notion of ``altered environment" of indirect intervention. 
From this point, we will use the terms ``option" and ``environment-aware option" interchangeably. 

We use the notion of environment-aware option to formally describe the two types of intervention. 
A direct intervention represents an option $(\mathcal{E}_{\tau}, \mathcal{I}, \pi_{\Phi}, \beta_{\Phi})$.
The option acts on the original task environment $\mathcal{E}_{\tau}$. 
The assistant's execution policy $\pi_{\Phi}$ serves as the acting policy and the assistant's termination functions decides when the intervention halts. 
On the other hand, an indirect intervention features an option $(\mathcal{E}_{\Phi(z, \tau)}, \mathcal{I}, \pi, \beta)$.
$\mathcal{E}_{\Phi(z, \tau)}$ is the task environment altered by the assistant given observation $z$ and task $\tau$.
The agent uses its own policies $\pi$ and $\beta$ rather than the assistant's policies to act.
Here, we assume that $\pi$ and $\beta$ is unaffected by the change of observation space, as in practice, we train them to make decisions under observation spaces of the altered environments.

\subsection{The Three Fundamental Problems in Leveraging Human Assistance}



